Probabilistic Counters for Privacy Preserving Data Aggregation

Probabilistic counters are well-known tools often used for space-efficient set cardinality estimation. In this paper, we investigate probabilistic counters from the perspective of preserving privacy. We use the standard, rigid differential privacy notion. The intuition is that the probabilistic counters do not reveal too much information about individuals but provide only general information about the population. Therefore, they can be used safely without violating the privacy of individuals. However, it turned out, that providing a precise, formal analysis of the privacy parameters of probabilistic counters is surprisingly difficult and needs advanced techniques and a very careful approach. We demonstrate that probabilistic counters can be used as a privacy protection mechanism without extra randomization. Namely, the inherent randomization from the protocol is sufficient for protecting privacy, even if the probabilistic counter is used multiple times. In particular, we present a specific privacy-preserving data aggregation protocol based on Morris Counter and MaxGeo Counter. Some of the presented results are devoted to counters that have not been investigated so far from the perspective of privacy protection. Another part is an improvement of previous results. We show how our results can be used to perform distributed surveys and compare the properties of counter-based solutions and a standard Laplace method.

==> commands.tex <==
\newcommand{\papertitle}{Oblivious Probabilistic Counters for Distributed Privacy Preserving Data Aggregation}
\newcommand{\shortpapertitle}{}



\makeatletter
\newlength\min@xx
\newcommand*\xxrightarrow[1]{\begingroup
  \settowidth\min@xx{$\m@th\scriptstyle#1$}
  \@xxrightarrow}
\newcommand*\@xxrightarrow[2][]{
  \sbox8{$\m@th\scriptstyle#1$}  % subscript
  \ifdim\wd8>\min@xx \min@xx=\wd8 \fi
  \sbox8{$\m@th\scriptstyle#2$} % superscript
  \ifdim\wd8>\min@xx \min@xx=\wd8 \fi
  \xrightarrow[{\mathmakebox[\min@xx]{\scriptstyle#1}}]
    {\mathmakebox[\min@xx]{\scriptstyle#2}}
  \endgroup}
\newcommand*\xxleftarrow[1]{\begingroup
  \settowidth\min@xx{$\m@th\scriptstyle#1$}
  \@xxleftarrow}
\newcommand*\@xxleftarrow[2][]{
  \sbox8{$\m@th\scriptstyle#1$}  % subscript
  \ifdim\wd8>\min@xx \min@xx=\wd8 \fi
  \sbox8{$\m@th\scriptstyle#2$} % superscript
  \ifdim\wd8>\min@xx \min@xx=\wd8 \fi
  \xleftarrow[{\mathmakebox[\min@xx]{\scriptstyle#1}}]
    {\mathmakebox[\min@xx]{\scriptstyle#2}}
  \endgroup}

\newcommand{\sect}[1]{\mbox{Sect.\,\ref{#1}}}  %cytowanie section w srodku zdania
\newcommand{\subsect}[1]{\mbox{Subsect.\,\ref{#1}}}  %cytowanie subsection w srodku zdania



\newcommand{\sign}{\mbox{sign}}
\newcommand{\nazwa}{CTRL-Sign}
\newcommand{\xor}{\oplus}
\newcommand{\RAND}{\textrm{RAND}}


%\usepackage{framed}
\usepackage{xcolor}


%%new left margin line
%\renewenvironment{leftbar}[1][\hsize]
%{%
    %\def\FrameCommand
    %{%
        %{\color{red}\vrule width 3pt}%
        %\hspace{6pt}%must no space.
        %%\fboxsep=\FrameSep\colorbox{blue}%
    %}%
    %\MakeFramed{\hsize#1\advance\hsize-\width\FrameRestore}%
%}
%{\endMakeFramed}

%renew paragraph
%\makeatletter
%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
  %{-3.25ex\@plus -1ex \@minus -.2ex}%
  %{1.5ex \@plus .2ex}%
  %{\normalfont\normalsize\bfseries}}
%\makeatother
%
%
%%new left margin line
%\renewenvironment{leftbar}[1][\hsize]
%{%
    %\def\FrameCommand
    %{%
        %{\color{red}\vrule width 3pt}%
        %\hspace{6pt}%must no space.
        %%\fboxsep=\FrameSep\colorbox{blue}%
    %}%
    %\MakeFramed{\hsize#1\advance\hsize-\width\FrameRestore}%
%}
%{\endMakeFramed}

%renew paragraph
%\makeatletter
%\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
  %{-3.25ex\@plus -1ex \@minus -.2ex}%
  %{1.5ex \@plus .2ex}%
  %{\normalfont\normalsize\bfseries}}
%\makeatother
%
%%note
%\renewenvironment{note}[1]{\begin{leftbar} \textbf{Note:} #1}{\end{leftbar}}

\newcommand{\Zp}{\mathbb{Z}_p}
\newcommand{\Fp}{\mathbb{F}_p}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\RR}{\mathbf{R}}
\newcommand{\ee}{\mathbf{e}}
\newcommand{\zz}{\mathbf{z}}
%\newcommand{\vv}{\mathbf{v}}
\newcommand{\wt}[1]{\mathbf{wt}\left({#1} \right) }
\newcommand{\EE}[1]{\mathbb{E}\left(#1\right)}
\newcommand{\PR}[1]{\mathbb{P}\left( #1 \right)}
% Morris counter
\newcommand{\Mor}{\mathrm{Mor}}
\newcommand{\ls}{\leqslant}
\newcommand{\gs}{\geqslant}
\newcommand{\WM}{\stackrel{W}{=}}
\newcommand{\eqthr}{\stackrel{(\ref{eq:base})}{=}}
%\DeclareMathOperator{\Ber}{Ber}
%\DeclareMathOperator{\log}{log}
%\DeclareMathOperator{\Pr}{Pr}
%\DeclareMathOperator{\ln}{ln}

\newcommand{\user}{\mathcal{U}}
\newcommand{\reader}{\mathcal{R}}
\newcommand{\rfid}{\mathcal{T}_{\user}}
\newcommand{\rfiddwa}{\mathcal{TS}_{\user}}
\newcommand{\PRNG}{\mathrm{prng}}
\newcommand{\Exp}{\textrm{E}}
\newcommand{\COMM}{\mathrm{cmt}}
\newcommand{\aspaceTR}{\aaa^{SPACEAA}_{TR}}

\newcommand{\data}{\mathcal{D}}
\newcommand{\smart}{\mathcal{S}_{\user}}
\newcommand{\manu}{\mathcal M}
\newcommand{\adver}{\mathcal A}
\newcommand{\prov}[2]{\mathcal P_{{#1},{#2}}}
\newcommand{\ver}[2]{\mathcal V_{{#1},{#2}}}
\newcommand{\prover}{\mathcal P}
\newcommand{\verifier}{\mathcal V}
\newcommand{\aaa}{\mathcal{A}}
\newcommand{\aaaa}{\mathcal{A}^{Auth}_A}
\newcommand{\aaap}{\mathcal{A}^{PFS}}
\DeclareMathOperator{\Ber}{Ber}
\DeclareMathOperator{\bigO}{O}
\DeclareMathOperator{\smallO}{o}
\newcommand{\E}[1]{E\left[#1\right]}
\newcommand{\var}[1]{\vvv \left[#1\right]}
\newcommand{\SmallO}[1]{\smallO\left(#1\right)}
\newcommand{\BigO}[1]{\bigO\left(#1\right)}
\DeclareMathOperator{\vvv}{var}
\newcommand{\len}[1]{\mathrm{length\left(#1\right)}}
\newcommand{\hash}{\mathcal{H}}
%%%%%%%%%%%%%%%%%%%%%%%%%
%Adversary&Nodes
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\AAA}{\mathcal{A}}
\newcommand{\Adv}{\mathrm{\mathbf{Adv}}}
\newcommand{\adv}{\mathrm{\mathbf{Adv}}}
\newcommand{\Node}{\mathrm{\mathbf{N}}}
\newcommand{\Agg}{\mathrm{\mathbf{AGG}}}
\newcommand{\lAgg}{\mathrm{\mathbf{Agg}}}
%%%%%%%%%%%%%%%%%%%%%%%%%
% Key pools
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\KeyPool}{\mathcal{K}}
\newcommand{\nKeyPool}[1]{\mathcal{K}^{\left( #1 \right)}}
\newcommand{\Key}[1]{\mathbf{K}_{#1}}
\newcommand{\nKey}[2]{\mathbf{K}_{#2}^{\left( #1 \right)}} %\nKey{nodeID}{keyNo}
%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ID}[1]{\mathrm{ID}\left( #1 \right)}
\newcommand{\Enc}[2]{\mathrm{Enc_{#1}\left( #2\right)}}
\newcommand{\Dec}[2]{\mathrm{Dec_{#1}\left( #2\right)}}
\newcommand{\sk}{\mathrm{sk}}
\newcommand{\ddh}{\mathrm{DDH}}
\newcommand{\enc}{\mathrm{ENC}}
\newcommand{\aspaceTF}{\mathcal{V}^{SPACEAA}_{TF}}

\newcommand{\alphaR}{\mathbf{R\_\alpha}}
\newcommand{\betaR}{\mathbf{R\_\beta}}

\newcommand{\true}{'1'}
\newcommand{\false}{'0'}

%\newtheorem{assumption}[theorem]{Assumption}
%\newtheorem{fact}[theorem]{Fact}

\newcommand{\kgr}[1]{$\triangleleft$\marginpar{\footnotesize{K:#1}}}
\newcommand{\Marek}[1]{$\triangleleft$\marginpar{\footnotesize{Marek:#1}}}

%correction: comment, old, new
\newcommand{\corr}[3]{{\color{red}#2}\, {\color{teal}#3}}
\newcommand{\ok}{\marginpar{\color{green}\checkmark}}
\newcommand{\no}{\marginpar{\color{red}\ding{55}}}

\newcommand{\cert}{\textit{cert}}
\newcommand{\xxxx}[1]{\marginpar{\footnotesize\checkmark #1}}
\newcommand{\extra}[2]{#2}

